Understanding Silent Failures in Medical Image Classification

To ensure the reliable use of classification systems in medical applications, it is crucial to prevent silent failures. This can be achieved by either designing classifiers that are robust enough to avoid failures in the first place, or by detecting remaining failures using confidence scoring functions (CSFs). A predominant source of failures in image classification is distribution shifts between training data and deployment data. To understand the current state of silent failure prevention in medical imaging, we conduct the first comprehensive analysis comparing various CSFs in four biomedical tasks and a diverse range of distribution shifts. Based on the result that none of the benchmarked CSFs can reliably prevent silent failures, we conclude that a deeper understanding of the root causes of failures in the data is required. To facilitate this, we introduce SF-Visuals, an interactive analysis tool that uses latent space clustering to visualize shifts and failures. On the basis of various examples, we demonstrate how this tool can help researchers gain insight into the requirements for safe application of classification systems in the medical domain. The open-source benchmark and tool are at: https://github.com/IML-DKFZ/sf-visuals.

==> tables/paper_results_condensed_accuracy.tex <==
\begin{tabular}{l?rrr?rrrr?rrr?rrr}
Dataset & \multicolumn{3}{c}{Chest X-ray} & \multicolumn{4}{c}{Dermoscopy} & \multicolumn{3}{c}{FC-Microscopy} & \multicolumn{3}{c}{Lung Nodule CT} \\
Study & iid & cor & acq & iid & cor & acq & man & iid & cor & acq & iid & cor & man \\
\midrule
MSR & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 66.2 & {\cellcolor[HTML]{FDA25A}} \color[HTML]{000000} 62.9 & {\cellcolor[HTML]{FDC794}} \color[HTML]{000000} 58.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 93.4 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 94.5 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 42.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 63.2 & {\cellcolor[HTML]{C64102}} \color[HTML]{F1F1F1} 28.0 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 39.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 82.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 81.3 & {\cellcolor[HTML]{FDD5AD}} \color[HTML]{000000} 78.1 \\
PE & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 66.2 & {\cellcolor[HTML]{FDA25A}} \color[HTML]{000000} 62.9 & {\cellcolor[HTML]{FDC794}} \color[HTML]{000000} 58.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 93.4 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 94.5 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 42.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 63.2 & {\cellcolor[HTML]{C64102}} \color[HTML]{F1F1F1} 28.0 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 39.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 82.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 81.3 & {\cellcolor[HTML]{FDD5AD}} \color[HTML]{000000} 78.1 \\
MCD-MSR & {\cellcolor[HTML]{F98230}} \color[HTML]{F1F1F1} 66.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 63.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 59.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 93.4 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 94.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 42.4 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 63.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 27.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 39.4 & {\cellcolor[HTML]{F36E19}} \color[HTML]{F1F1F1} 84.4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 83.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 79.1 \\
MCD-PE & {\cellcolor[HTML]{F98230}} \color[HTML]{F1F1F1} 66.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 63.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 59.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 93.4 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 94.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 42.4 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 63.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 27.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 39.4 & {\cellcolor[HTML]{F36E19}} \color[HTML]{F1F1F1} 84.4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 83.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 79.1 \\
MCD-EE & {\cellcolor[HTML]{F98230}} \color[HTML]{F1F1F1} 66.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 63.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 59.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 93.4 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 94.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 42.4 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 63.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 27.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 39.4 & {\cellcolor[HTML]{F36E19}} \color[HTML]{F1F1F1} 84.4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 83.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 79.1 \\
ConfidNet & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 66.2 & {\cellcolor[HTML]{FDA25A}} \color[HTML]{000000} 62.9 & {\cellcolor[HTML]{FDC794}} \color[HTML]{000000} 58.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 94.7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 93.4 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 94.5 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 42.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 63.2 & {\cellcolor[HTML]{C64102}} \color[HTML]{F1F1F1} 28.0 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 39.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 82.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 81.3 & {\cellcolor[HTML]{FDD5AD}} \color[HTML]{000000} 78.1 \\
DG-MCD-MSR & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 67.5 & {\cellcolor[HTML]{FDB06E}} \color[HTML]{000000} 63.0 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 57.8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 94.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 93.6 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 94.9 & {\cellcolor[HTML]{8A2B04}} \color[HTML]{F1F1F1} 39.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 71.6 & {\cellcolor[HTML]{FDA45D}} \color[HTML]{000000} 29.3 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 39.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 88.1 & {\cellcolor[HTML]{FDA159}} \color[HTML]{000000} 83.2 & {\cellcolor[HTML]{FDCB9B}} \color[HTML]{000000} 77.9 \\
DG-RES & {\cellcolor[HTML]{E45709}} \color[HTML]{F1F1F1} 66.6 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 61.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 55.3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 94.5 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 93.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 95.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 39.7 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 71.1 & {\cellcolor[HTML]{FDD8B2}} \color[HTML]{000000} 30.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 38.8 & {\cellcolor[HTML]{FEE0C1}} \color[HTML]{000000} 87.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 84.6 & {\cellcolor[HTML]{FC8A39}} \color[HTML]{F1F1F1} 76.8 \\
Devries et al. & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 67.5 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 63.4 & {\cellcolor[HTML]{FDA45D}} \color[HTML]{000000} 58.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 93.5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 93.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 93.9 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 39.9 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 71.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 30.7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 39.2 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 87.7 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 84.5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 74.6 \\
\bottomrule
\end{tabular}

==> tables/paper_results_condensed_b-accuracy.tex <==
\begin{tabular}{l?rrr?rrrr?rrr?rrr}
Dataset & \multicolumn{3}{c}{Chest X-ray} & \multicolumn{4}{c}{Dermoscopy} & \multicolumn{3}{c}{FC-Microscopy} & \multicolumn{3}{c}{Lung Nodule CT} \\
Study & iid & cor & acq & iid & cor & acq & man & iid & cor & acq & iid & cor & man \\
\midrule
MSR & {\cellcolor[HTML]{EB600E}} \color[HTML]{F1F1F1} 36.5 & {\cellcolor[HTML]{F16913}} \color[HTML]{F1F1F1} 33.3 & {\cellcolor[HTML]{FD9B50}} \color[HTML]{000000} 34.3 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 87.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 62.7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 60.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 62.9 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 27.3 & {\cellcolor[HTML]{FD8C3B}} \color[HTML]{F1F1F1} 37.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 85.0 & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 82.4 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 74.2 \\
PE & {\cellcolor[HTML]{EB600E}} \color[HTML]{F1F1F1} 36.5 & {\cellcolor[HTML]{F16913}} \color[HTML]{F1F1F1} 33.3 & {\cellcolor[HTML]{FD9B50}} \color[HTML]{000000} 34.3 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 87.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 62.7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 60.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 62.9 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 27.3 & {\cellcolor[HTML]{FD8C3B}} \color[HTML]{F1F1F1} 37.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 85.0 & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 82.4 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 74.2 \\
MCD-MSR & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 34.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 31.6 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 32.7 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 87.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 62.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 60.4 & {\cellcolor[HTML]{942F03}} \color[HTML]{F1F1F1} 63.5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 26.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 38.2 & {\cellcolor[HTML]{D94801}} \color[HTML]{F1F1F1} 85.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 82.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 74.7 \\
MCD-PE & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 34.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 31.6 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 32.7 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 87.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 62.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 60.4 & {\cellcolor[HTML]{942F03}} \color[HTML]{F1F1F1} 63.5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 26.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 38.2 & {\cellcolor[HTML]{D94801}} \color[HTML]{F1F1F1} 85.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 82.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 74.7 \\
MCD-EE & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 34.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 31.6 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 32.7 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 87.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 62.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 60.4 & {\cellcolor[HTML]{942F03}} \color[HTML]{F1F1F1} 63.5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 26.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 38.2 & {\cellcolor[HTML]{D94801}} \color[HTML]{F1F1F1} 85.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 82.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 74.7 \\
ConfidNet & {\cellcolor[HTML]{EB600E}} \color[HTML]{F1F1F1} 36.5 & {\cellcolor[HTML]{F16913}} \color[HTML]{F1F1F1} 33.3 & {\cellcolor[HTML]{FD9B50}} \color[HTML]{000000} 34.3 & {\cellcolor[HTML]{952F03}} \color[HTML]{F1F1F1} 87.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 62.7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 60.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 62.9 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 27.3 & {\cellcolor[HTML]{FD8C3B}} \color[HTML]{F1F1F1} 37.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 85.0 & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 82.4 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 74.2 \\
DG-MCD-MSR & {\cellcolor[HTML]{FDB77A}} \color[HTML]{000000} 38.1 & {\cellcolor[HTML]{FDA159}} \color[HTML]{000000} 34.2 & {\cellcolor[HTML]{D54601}} \color[HTML]{F1F1F1} 33.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 86.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 80.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 58.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 59.2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 71.5 & {\cellcolor[HTML]{FD984B}} \color[HTML]{000000} 28.5 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 37.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 87.8 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 81.4 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 74.2 \\
DG-RES & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 39.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 36.1 & {\cellcolor[HTML]{FD9B50}} \color[HTML]{000000} 34.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 86.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 80.9 & {\cellcolor[HTML]{862A04}} \color[HTML]{F1F1F1} 59.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 59.2 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 71.1 & {\cellcolor[HTML]{FDCFA0}} \color[HTML]{000000} 29.2 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 37.6 & {\cellcolor[HTML]{FEDDBC}} \color[HTML]{000000} 87.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 80.6 & {\cellcolor[HTML]{FB8634}} \color[HTML]{F1F1F1} 72.6 \\
Devries et al. & {\cellcolor[HTML]{FEE7D0}} \color[HTML]{000000} 39.2 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 35.2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 35.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 88.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{C84202}} \color[HTML]{F1F1F1} 59.7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 59.2 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 71.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 30.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 38.2 & {\cellcolor[HTML]{FDD7AF}} \color[HTML]{000000} 87.2 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 70.7 \\
\bottomrule
\end{tabular}

==> tables/paper_results_condensed_failauc.tex <==
\begin{tabular}{l?rrr?rrrr?rrr?rrr}
Dataset & \multicolumn{3}{c}{Chest X-ray} & \multicolumn{4}{c}{Dermoscopy} & \multicolumn{3}{c}{FC-Microscopy} & \multicolumn{3}{c}{Lung Nodule CT} \\
Study & iid & cor & acq & iid & cor & acq & man & iid & cor & acq & iid & cor & man \\
\midrule
MSR & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 77.0 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 77.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 93.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 91.3 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 90.6 & {\cellcolor[HTML]{DF5106}} \color[HTML]{F1F1F1} 55.1 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 86.6 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{EF6612}} \color[HTML]{F1F1F1} 78.7 & {\cellcolor[HTML]{FDCD9C}} \color[HTML]{000000} 75.8 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 70.5 \\
PE & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 78.5 & {\cellcolor[HTML]{FEECD9}} \color[HTML]{000000} 76.4 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 76.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 93.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 91.3 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 90.6 & {\cellcolor[HTML]{DF5106}} \color[HTML]{F1F1F1} 55.1 & {\cellcolor[HTML]{FDB678}} \color[HTML]{000000} 84.6 & {\cellcolor[HTML]{FEE4CA}} \color[HTML]{000000} 76.4 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{EF6612}} \color[HTML]{F1F1F1} 78.7 & {\cellcolor[HTML]{FDCD9C}} \color[HTML]{000000} 75.8 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 70.5 \\
MCD-MSR & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 77.3 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 77.0 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 93.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 91.3 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 90.6 & {\cellcolor[HTML]{DB4B03}} \color[HTML]{F1F1F1} 54.9 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000} 87.6 & {\cellcolor[HTML]{FFEFDF}} \color[HTML]{000000} 78.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 86.1 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 78.5 & {\cellcolor[HTML]{FDD6AE}} \color[HTML]{000000} 76.3 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 70.8 \\
MCD-PE & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 78.5 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 76.6 & {\cellcolor[HTML]{FEE5CC}} \color[HTML]{000000} 75.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 93.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 91.3 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 90.6 & {\cellcolor[HTML]{DB4B03}} \color[HTML]{F1F1F1} 54.9 & {\cellcolor[HTML]{FDC997}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{FEE5CB}} \color[HTML]{000000} 76.5 & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 85.6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 78.5 & {\cellcolor[HTML]{FDD6AE}} \color[HTML]{000000} 76.3 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 70.8 \\
MCD-EE & {\cellcolor[HTML]{FEE9D4}} \color[HTML]{000000} 78.5 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 76.6 & {\cellcolor[HTML]{FEE5CC}} \color[HTML]{000000} 75.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 93.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 91.3 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 90.6 & {\cellcolor[HTML]{DB4B03}} \color[HTML]{F1F1F1} 54.9 & {\cellcolor[HTML]{FDC997}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{FEE5CB}} \color[HTML]{000000} 76.5 & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 85.6 & {\cellcolor[HTML]{F67723}} \color[HTML]{F1F1F1} 79.1 & {\cellcolor[HTML]{FDD1A4}} \color[HTML]{000000} 76.0 & {\cellcolor[HTML]{FDDAB6}} \color[HTML]{000000} 69.7 \\
ConfidNet & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 79.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 77.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 77.2 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 92.8 & {\cellcolor[HTML]{FEE3C8}} \color[HTML]{000000} 90.4 & {\cellcolor[HTML]{FEECD9}} \color[HTML]{000000} 90.5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 51.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 73.9 & {\cellcolor[HTML]{A83703}} \color[HTML]{F1F1F1} 62.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 51.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 82.9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{DF5106}} \color[HTML]{F1F1F1} 65.1 \\
DG-MCD-MSR & {\cellcolor[HTML]{FFEEDE}} \color[HTML]{000000} 78.9 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 76.5 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 76.0 & {\cellcolor[HTML]{FEE3C8}} \color[HTML]{000000} 93.0 & {\cellcolor[HTML]{FFF3E7}} \color[HTML]{000000} 91.2 & {\cellcolor[HTML]{FEE2C6}} \color[HTML]{000000} 90.0 & {\cellcolor[HTML]{F9812E}} \color[HTML]{F1F1F1} 57.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 90.3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 84.8 & {\cellcolor[HTML]{FDB576}} \color[HTML]{000000} 80.6 & {\cellcolor[HTML]{FDC997}} \color[HTML]{000000} 75.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 71.4 \\
DG-RES & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 70.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 65.9 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 67.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 90.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 85.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 83.7 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 62.8 & {\cellcolor[HTML]{FDA863}} \color[HTML]{000000} 83.8 & {\cellcolor[HTML]{FDC895}} \color[HTML]{000000} 73.7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000} 77.4 & {\cellcolor[HTML]{DD4D04}} \color[HTML]{F1F1F1} 78.1 & {\cellcolor[HTML]{EA5F0E}} \color[HTML]{F1F1F1} 71.6 & {\cellcolor[HTML]{FDBA7F}} \color[HTML]{000000} 68.5 \\
Devries et al. & {\cellcolor[HTML]{FEE3C8}} \color[HTML]{000000} 78.1 & {\cellcolor[HTML]{FFEFDF}} \color[HTML]{000000} 76.7 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 76.9 & {\cellcolor[HTML]{FD9141}} \color[HTML]{000000} 91.8 & {\cellcolor[HTML]{FDCFA0}} \color[HTML]{000000} 89.7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 91.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 63.2 & {\cellcolor[HTML]{EB610F}} \color[HTML]{F1F1F1} 79.6 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 59.9 & {\cellcolor[HTML]{F06712}} \color[HTML]{F1F1F1} 64.4 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 76.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 68.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 62.6 \\
\bottomrule
\end{tabular}
